The sample complexity of multi-reference alignment

The growing role of data-driven approaches to scientific discovery has unveiled a large class of models that involve latent transformations with a rigid algebraic constraint. Three-dimensional molecule reconstruction in Cryo-Electron Microscopy (cryo-EM) is a central problem in this class. Despite decades of algorithmic and software development, there is still little theoretical understanding of the sample complexity of this problem, that is, number of images required for 3-D reconstruction. Here we consider multi-reference alignment (MRA), a simple model that captures fundamental aspects of the statistical and algorithmic challenges arising in cryo-EM and related problems. In MRA, an unknown signal is subject to two types of corruption: a latent cyclic shift and the more traditional additive white noise. The goal is to recover the signal at a certain precision from independent samples. While at high signal-to-noise ratio (SNR), the number of observations needed to recover a generic signal is proportional to $1/\mathrm{SNR}$, we prove that it rises to a surprising $1/\mathrm{SNR}^3$ in the low SNR regime. This precise phenomenon was observed empirically more than twenty years ago for cryo-EM but has remained unexplained to date. Furthermore, our techniques can easily be extended to the heterogeneous MRA model where the samples come from a mixture of signals, as is often the case in applications such as cryo-EM, where molecules may have different conformations. This provides a first step towards a statistical theory for heterogeneous cryo-EM.

==> arXiv version/commands.tex <==

\usepackage{amsmath, amssymb, color}
\usepackage{amsthm} 
%\usepackage{natbib}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
%
\RequirePackage{hypernat}
\usepackage{cleveref}
%
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
% \addto{\captionsamerican}{\renewcommand{\abstractname}{}}
%
\usepackage{psfrag,color}
\usepackage{dcolumn}
% \usepackage{subfigure}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}
\usepackage[final]{showkeys}
\renewcommand*\showkeyslabelformat[1]{%
\fbox{\normalfont\tiny\ttfamily#1}}


\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
%
%\usepackage{algorithmic, algorithm}
\usepackage{wrapfig}


\usepackage{amssymb, latexsym}

%
\usepackage{graphicx}
%
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

%% if you need to pass options to natbib, use, e.g.:
%% \PassOptionsToPackage{numbers, compress}{natbib}
%% before loading nips_2017
%%
%% to avoid loading the natbib package, add option nonatbib:
%%\usepackage[nonatbib]{nips_2017}
%
%%\usepackage[nonatbib]{nips_2017}
%
%% to compile a camera-ready version, replace the above line with the following, which has the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{wrapfig}        % for wrapping figures
%\usepackage[notref, notcite, final]{showkeys}
%
%\usepackage{amsmath, amsthm, amsfonts}
%\usepackage{dsfont}
%\usepackage[sort]{cite}
%\usepackage{graphicx}
%
%% Notes
\usepackage{color}
\newcommand{\jw}[1]{{\textcolor{red}{[\textbf{JON:} #1]}}}
%\newcommand{\pr}[1]{{\textcolor{blue}{[\textbf{PR:} #1]}}}
%
%% For algorithms
\usepackage{algorithm}
%%\usepackage[noend]{algorithmic}
\usepackage[noend]{algcompatible}
%
%% Theorem definitions
\newtheorem{defin}{Definition}%[section]
\newtheorem{thm}{Theorem}%[section]
\newtheorem{exe}{Exercise}%[section]
\newtheorem{exa}{Example}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corol}{Corollary}%[thm]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{discussion}{Discussion}%[section]
\newtheorem{conc}{Conclusion}%[section]

% Custom definitions

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%\renewcommand{\subseteq}{\subset}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand*{\ep}{\varepsilon}
\newcommand*{\defeq}{:=}
\newcommand*{\dd}{\,\mathrm{d}}



==> commands.tex <==

\usepackage{amsmath, amssymb, color}
\usepackage{amsthm} 
%\usepackage{natbib}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
%
\RequirePackage{hypernat}
\usepackage{cleveref}
%
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
% \addto{\captionsamerican}{\renewcommand{\abstractname}{}}
%
\usepackage{psfrag,color}
\usepackage{dcolumn}
% \usepackage{subfigure}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}
\usepackage[final]{showkeys}
\renewcommand*\showkeyslabelformat[1]{%
\fbox{\normalfont\tiny\ttfamily#1}}


\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
%
%\usepackage{algorithmic, algorithm}
\usepackage{wrapfig}


\usepackage{amssymb, latexsym}

%
\usepackage{graphicx}
%
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

%% if you need to pass options to natbib, use, e.g.:
%% \PassOptionsToPackage{numbers, compress}{natbib}
%% before loading nips_2017
%%
%% to avoid loading the natbib package, add option nonatbib:
%%\usepackage[nonatbib]{nips_2017}
%
%%\usepackage[nonatbib]{nips_2017}
%
%% to compile a camera-ready version, replace the above line with the following, which has the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{wrapfig}        % for wrapping figures
%\usepackage[notref, notcite, final]{showkeys}
%
%\usepackage{amsmath, amsthm, amsfonts}
%\usepackage{dsfont}
%\usepackage[sort]{cite}
%\usepackage{graphicx}
%
%% Notes
\usepackage{color}
\newcommand{\jw}[1]{{\textcolor{red}{[\textbf{JON:} #1]}}}
%\newcommand{\pr}[1]{{\textcolor{blue}{[\textbf{PR:} #1]}}}
%
%% For algorithms
\usepackage{algorithm}
%%\usepackage[noend]{algorithmic}
\usepackage[noend]{algcompatible}
%
%% Theorem definitions
\newtheorem{defin}{Definition}%[section]
\newtheorem{thm}{Theorem}%[section]
\newtheorem{exe}{Exercise}%[section]
\newtheorem{exa}{Example}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corol}{Corollary}%[thm]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{discussion}{Discussion}%[section]
\newtheorem{conc}{Conclusion}%[section]

% Custom definitions

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%\renewcommand{\subseteq}{\subset}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand*{\ep}{\varepsilon}
\newcommand*{\defeq}{:=}
\newcommand*{\dd}{\,\mathrm{d}}


